Rotating Isospectral Drums

In this thesis I demonstrate that isospectral domains, that is domains of differing geometric shapes that possess identical spectra, do not remain isospectral when subject to uniform rotation. One thus *can* hear the shape of a rotating drum. It is shown that the spectra diverge as $\propto\left(\frac{\omega}{c}\right)^2$ similarly to a square but different from a circle, whose degenerate eigenfrequencies split $\propto \left(\frac{\omega}{c}\right)$. The latter two cases are studied analytically and used as test cases for the selection of numerical solution methods. I demonstrate that the presence of a simple medium attenuates the effects of rotation on the spectrum differences. Further I show that the common but linearised augmented wave equation yields eigenmodes with sensible structure for non-physical parameters, whereas a full equation destroys the structure as intended. The full equation is obtained from first principles using Maxwell equations formulated as differential forms and a careful application of the 3+1 foliation of space-time. The differences of the result from literature arXiv:physics/0607016 are highlighted and their effects studied. The equation is treated analytically on simple domains to obtain reference data for numerical analysis. Nodal and modal discretisations of the PDE are tested and a self-written FEM implementation is chosen due to higher precision of the results. As part of the validation process I demonstrate that results of arXiv:physics/0607016 are reproducible. The resulting gyroscopic quadratic eigenvalue problem is linearised into a Hamiltonian/skew-Hamiltonian pencil and a suitable shift operator for the Arnoldi iteration is determined. The resulting formulation is solved using ARPACK.

==> simplify.tex <==
% (c) 2002 V. Schwamberger, last change: 02.11.2003
% pdfLaTeX - definitions of unions and other usefull things
%%%%%%%%%%%%%%%%%%%            HEADER            %%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{upgreek}

% change \varphi und \phi
%\DeclareMathSymbol{\varphi}{\mathord}{letters}{"1E}
%\DeclareMathSymbol{\phi}{\mathord}{letters}{"27}

%\pdfadjustspacing=2

% define \pdfproducer
\makeatletter
%\def\pdfproducer{pdfTeX}
%\ifx\pdftexversion\@undefined
%\else
%  \ifnum\pdftexversion<100 %
%    \edef\pdfproducer{%
%      \pdfproducer
%      \the\pdftexversion.\pdftexrevision
%    }
%  \else
%    \edef\pdfproducer{%
%      \pdfproducer-%
%      \expandafter\@car\the\pdftexversion\@empty\@nil.%
%      \expandafter\@cdr\the\pdftexversion\@empty\@nil
%      \pdftexrevision
%    }
%  \fi
%\fi
\def\pdfproducer{pdfTeX}
\ifx\eTeXversion\@undefined
\else
  \ifx\eTeXversion\relax
  \else
    \ifnum\eTeXversion>0 %
      \def\pdfproducer{pdfeTeX}
    \fi
  \fi
\fi
\ifx\pdftexversion\@undefined
\else
  \ifnum\pdftexversion<100 %
    \edef\pdfproducer{%
      \pdfproducer
      \the\pdftexversion.\pdftexrevision
    }
  \else
    \edef\pdfproducer{%
      \pdfproducer-%
      \expandafter\@car\the\pdftexversion\@empty\@nil.%
      \expandafter\@cdr\the\pdftexversion\@empty\@nil
      \pdftexrevision
    }
  \fi
\fi
\makeatother

%Abkürzungen für die Quantenmechanik: DIRAC-Notation
\newcommand{\bra}[1]{\ensuremath{\langle #1|}}
\newcommand{\ket}[1]{\ensuremath{|#1\rangle}}
\newcommand{\brak}[2]{\ensuremath{\langle #1|#2\rangle}}
\newcommand{\avge}[1]{\ensuremath{\langle #1\rangle}}

% with \left .. \right
\newcommand{\dbra}[1]{\ensuremath{\left\langle #1\right|}}
\newcommand{\dket}[1]{\ensuremath{\left|#1\right\rangle}}
\newcommand{\dbrak}[2]{\ensuremath{\left\langle #1\right|\left.#2\right\rangle}}
\newcommand{\davge}[1]{\ensuremath{\left\langle #1\right\rangle}}

\newcommand{\fbra}[1]{\ensuremath{\left\langle \textstyle #1\right|}}
\newcommand{\fket}[1]{\ensuremath{\left|\textstyle #1\right\rangle}}
\newcommand{\fbrak}[2]{\ensuremath{\left\langle \textstyle #1\right|\left.\textstyle #2\right\rangle}}

% Abkürzungen für die Mathematik
\newcommand{\diag}{\operatorname{diag}}
\newcommand{\lint}{\int\limits}     % Integralgrenzen oben und unten
\newcommand{\e}{\mathrm{e}}
\newcommand{\down}[2]{\overset{\overset{\text{#1}}{\downarrow}}{#2}}
\newcommand{\adown}[2]{\overset{\makebox[0pt]{$\overset{\text{\tiny #1}}{\downarrow}$}}{#2}}
\newcommand{\ddown}[3]{\overset{\overset{\overset{\text{#1}}{\text{\tiny #2}}}{\downarrow}}{#3}}
\newcommand{\addown}[3]{\overset{\overset{\makebox[0pt]{$\overset{\text{\tiny #1}}{\text{\tiny #2}}$}}{\downarrow}}{#3}}

% Mathematical operators not present in AMSMATH
\DeclareMathOperator{\artanh}{artanh} %area-tangens hyperbolicus
\DeclareMathOperator{\arsinh}{arsinh} %area sinus-hyperbolicus
\DeclareMathOperator{\supp}{supp}	%support of a function
\newcommand{\sgn}{\text{sgn}}		%sign function

% Zahlenräume
\newcommand{\NN}{\mathbb{N}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\KK}{\mathbb{K}}
\newcommand{\RRon}[1]{\mathbb{R}^{#1}\backslash \{0\}}

% Vektoranalysis
\newcommand{\ds}{d\vec{s}}
\newcommand{\dob}{d\vec{o}}
\newcommand{\del}{\partial}
\newcommand{\ddel}[1]{\frac{\del}{\del #1}}
\newcommand{\deldel}[2]{\frac{\del #1}{\del #2}}

% Differential geometry
\newcommand{\Mf}{\mathcal{M}}	%Manifold
\newcommand{\Nf}{\mathcal{N}}	%Manifold
\newcommand{\CF}{\mathcal{F}}	%Faraday 2-form
\newcommand{\CJ}{\mathcal{J}}	%Current 1-form
\newcommand{\Tf}[3]{\mathcal{T}^{#1}_{#2}\left(#3\right)} %T^1_2 (3) Tensorfield
\newcommand{\IP}[3]{\langle #1\vert #2\rangle_{#3}}			%Inner product
\newcommand{\CalB}{\mathcal{B}}	%Magnetic field 2-form
\newcommand{\CalD}{\mathcal{D}}	%Electric excitation 2-form
\newcommand{\CalH}{\mathcal{H}}	%Magnetic excitation 1-form


% Nablaoperatoren
\newcommand{\grad}{\operatorname{grad}} % grad
\newcommand{\divv}{\operatorname{div}}  % div
\newcommand{\rot}{\operatorname{rot}}   % rot

% Funktionentheorie
\newcommand{\Res}{\operatorname{Res}}   % Residuum
\newcommand{\sign}{\operatorname{sign}} % Signum

% Abkürzungen für die Physik
% Volumen
\newcommand{\li}{\operatorname{l}}      % l
\newcommand{\mli}{\operatorname{ml}}    % ml

% Länge
\newcommand{\km}{\operatorname{km}}     % km
\newcommand{\m}{\operatorname{m}}       % m
\newcommand{\cm}{\operatorname{cm}}     % cm
\newcommand{\mm}{\operatorname{mm}}     % mm
\newcommand{\mum}{\operatorname{\upmu m}}% µm
\newcommand{\nm}{\operatorname{nm}}     % nm
\newcommand{\fm}{\operatorname{fm}}     % fm

% Kraft
\newcommand{\kN}{\operatorname{kN}}     % kN
\newcommand{\N}{\operatorname{N}}       % N
\newcommand{\mN}{\operatorname{mN}}     % mN

% Masse
\newcommand{\kg}{\operatorname{kg}}     % kg
\newcommand{\g}{\operatorname{g}}       % g
\newcommand{\mg}{\operatorname{mg}}     % mg
\newcommand{\um}{\operatorname{u}}      % u

% Anzahl
\newcommand{\mol}{\operatorname{mol}}   % mol

% Volt
\newcommand{\kV}{\operatorname{kV}}     % kV
\newcommand{\V}{\operatorname{V}}       % V
\newcommand{\mV}{\operatorname{mV}}     % mV
\newcommand{\muV}{\operatorname{\upmu V}}% µV

% Strom
\newcommand{\A}{\operatorname{A}}       % A
\newcommand{\mA}{\operatorname{mA}}     % mA
\newcommand{\muA}{\operatorname{\upmu A}}% µA
\newcommand{\nA}{\operatorname{nA}}     % nA

% Ladung
\newcommand{\C}{\operatorname{C}}       % C
\newcommand{\mC}{\operatorname{mC}}     % mC

% Frequenz
\newcommand{\Hz}{\operatorname{Hz}}     % Hz
\newcommand{\kHz}{\operatorname{kHz}}   % kHz
\newcommand{\MHz}{\operatorname{MHz}}   % MHz
\newcommand{\GHz}{\operatorname{GHz}}   % GHz

% Zeit
\newcommand{\s}{\operatorname{s}}       % s
\newcommand{\ms}{\operatorname{ms}}     % ms
\newcommand{\mus}{\operatorname{\upmu s}}% µs
\newcommand{\ns}{\operatorname{ns}}     % ns

% B-Feld
\newcommand{\Wb}{\operatorname{Wb}}     % Wb := Webern
\newcommand{\T}{\operatorname{T}}       % T
\newcommand{\mT}{\operatorname{mT}}     % mT
\newcommand{\muT}{\operatorname{\upmu T}}% µT

% Leistung
\newcommand{\W}{\operatorname{W}}       % W
\newcommand{\mW}{\operatorname{mW}}     % mW

% Arbeit
\newcommand{\J}{\operatorname{J}}       % J
\newcommand{\kJ}{\operatorname{kJ}}     % kJ
\newcommand{\eV}{\operatorname{eV}}     % eV
\newcommand{\keV}{\operatorname{keV}}   % keV
\newcommand{\MeV}{\operatorname{MeV}}   % MeV
\newcommand{\GeV}{\operatorname{GeV}}   % GeV

% Widerstand
\newcommand{\Ohm}{\Omega}                 % Ohm
\newcommand{\kOhm}{\operatorname{k\Omega}}% kOhm
\newcommand{\MOhm}{\operatorname{M\Omega}}% MOhm

% Kapazität
\newcommand{\F}{\operatorname{F}}       % F
\newcommand{\mF}{\operatorname{mF}}     % mF
\newcommand{\muF}{\operatorname{\upmu F}}% µF
\newcommand{\nF}{\operatorname{nF}}     % nF

% Druck
\newcommand{\bbar}{\operatorname{bar}}      % bar
\newcommand{\mbar}{\operatorname{mbar}}     % mbar
\newcommand{\mubar}{\operatorname{\upmu bar}}% µbar
\newcommand{\nbar}{\operatorname{nbar}}     % nbar
\newcommand{\Pa}{\operatorname{Pa}}         % Pa

% Induktivität
\newcommand{\He}{\operatorname{H}}      % H
\newcommand{\mgH}{\operatorname{mH}}     % mH

% Aktivität
\newcommand{\Bq}{\operatorname{Bq}}     % Bq

% Temperatur
\newcommand{\K}{\operatorname{K}}       % K

% Abkürzungen für die Informatik
\newcommand{\B}{\operatorname{B}}       % B := Bytes
\newcommand{\kB}{\operatorname{kiB}}     % kB
\newcommand{\MB}{\operatorname{MiB}}     % MB
\newcommand{\GB}{\operatorname{GiB}}     % GB
\newcommand{\TB}{\operatorname{TiB}}     % TB
\newcommand{\bi}{\operatorname{b}}      % b := bits
\newcommand{\kb}{\operatorname{kib}}     % kb
\newcommand{\Mb}{\operatorname{Mib}}     % Mb

\newcommand{\cost}{\operatorname{cost}} % cost()-Funktion
\newcommand{\dist}{\operatorname{dist}} % dist()-Funktion


% Fette Kleinbuchstaben (fuer Vektoren)

\newcommand{\Va}{{\mathbf{a}}}
\newcommand{\Vb}{{\mathbf{b}}}
\newcommand{\Vc}{{\mathbf{c}}}
\newcommand{\Vd}{{\mathbf{d}}}
\newcommand{\Ve}{{\mathbf{e}}}
\newcommand{\Vf}{{\mathbf{f}}}
\newcommand{\Vg}{{\mathbf{g}}}
\newcommand{\Vh}{{\mathbf{h}}}
\newcommand{\Vi}{{\mathbf{i}}}
\newcommand{\Vj}{{\mathbf{j}}}
\newcommand{\Vk}{{\mathbf{k}}}
\newcommand{\Vl}{{\mathbf{l}}}
\newcommand{\Vm}{{\mathbf{m}}}
\newcommand{\Vn}{{\mathbf{n}}}
\newcommand{\Vo}{{\mathbf{o}}}
\newcommand{\Vp}{{\mathbf{p}}}
\newcommand{\Vq}{{\mathbf{q}}}
\newcommand{\Vr}{{\mathbf{r}}}
\newcommand{\Vs}{{\mathbf{s}}}
\newcommand{\Vt}{{\mathbf{t}}}
\newcommand{\Vu}{{\mathbf{u}}}
\newcommand{\Vv}{{\mathbf{v}}}
\newcommand{\Vw}{{\mathbf{w}}}
\newcommand{\Vx}{{\mathbf{x}}}
\newcommand{\Vy}{{\mathbf{y}}}
\newcommand{\Vz}{{\mathbf{z}}}

%Small bold characters with hat on top

\newcommand{\VaH}{\widehat{\mathbf{a}}}
\newcommand{\VbH}{\widehat{\mathbf{b}}}
\newcommand{\VcH}{\widehat{\mathbf{c}}}
\newcommand{\VdH}{\widehat{\mathbf{d}}}
\newcommand{\VeH}{\widehat{\mathbf{e}}}
\newcommand{\VfH}{\widehat{\mathbf{f}}}
\newcommand{\VgH}{\widehat{\mathbf{g}}}
\newcommand{\VhH}{\widehat{\mathbf{h}}}
\newcommand{\ViH}{\widehat{\boldsymbol \imath}}
\newcommand{\VjH}{\widehat{\boldsymbol \jmath}}
\newcommand{\VkH}{\widehat{\mathbf{k}}}
\newcommand{\VlH}{\widehat{\mathbf{l}}}
\newcommand{\VmH}{\widehat{\mathbf{m}}}
\newcommand{\VnH}{\widehat{\mathbf{n}}}
\newcommand{\VoH}{\widehat{\mathbf{o}}}
\newcommand{\VpH}{\widehat{\mathbf{p}}}
\newcommand{\VqH}{\widehat{\mathbf{q}}}
\newcommand{\VrH}{\widehat{\mathbf{r}}}
\newcommand{\VsH}{\widehat{\mathbf{s}}}
\newcommand{\VtH}{\widehat{\mathbf{t}}}
\newcommand{\VuH}{\widehat{\mathbf{u}}}
\newcommand{\VvH}{\widehat{\mathbf{v}}}
\newcommand{\VwH}{\widehat{\mathbf{w}}}
\newcommand{\VxH}{\widehat{\mathbf{x}}}
\newcommand{\VyH}{\widehat{\mathbf{y}}}
\newcommand{\VzH}{\widehat{\mathbf{z}}}

%Small  characters with hat on top

\newcommand{\aH}{\widehat{ {a}}}
\newcommand{\bH}{\widehat{ {b}}}
\newcommand{\cH}{\widehat{ {c}}}
\newcommand{\dH}{\widehat{ {d}}}
\newcommand{\eH}{\widehat{ {e}}}
\newcommand{\fH}{\widehat{ {f}}}
\newcommand{\gH}{\widehat{ {g}}}
\newcommand{\hH}{\widehat{ {h}}}
\newcommand{\iH}{\widehat{ \imath}}
\newcommand{\jH}{\widehat{ \jmath}}
\newcommand{\kH}{\widehat{ {k}}}
\newcommand{\lH}{\widehat{ {l}}}
\newcommand{\mH}{\widehat{ {m}}}
\newcommand{\nH}{\widehat{ {n}}}
\newcommand{\oH}{\widehat{ {o}}}
\newcommand{\pH}{\widehat{ {p}}}
\newcommand{\qH}{\widehat{ {q}}}
\newcommand{\rH}{\widehat{ {r}}}
\newcommand{\sH}{\widehat{ {s}}}
\newcommand{\tH}{\widehat{ {t}}}
\newcommand{\uH}{\widehat{ {u}}}
\newcommand{\vH}{\widehat{ {v}}}
\newcommand{\wH}{\widehat{ {w}}}
\newcommand{\xH}{\widehat{ {x}}}
\newcommand{\yH}{\widehat{ {y}}}
\newcommand{\zH}{\widehat{ {z}}}


%Small bold characters with arrow on top

\newcommand{\Vax}{\vec{\mathbf{a}}}
\newcommand{\Vbx}{\vec{\mathbf{b}}}
\newcommand{\Vcx}{\vec{\mathbf{c}}}
\newcommand{\Vdx}{\vec{\mathbf{d}}}
\newcommand{\Vex}{\vec{\mathbf{e}}}
\newcommand{\Vfx}{\vec{\mathbf{f}}}
\newcommand{\Vgx}{\vec{\mathbf{g}}}
\newcommand{\Vhx}{\vec{\mathbf{h}}}
\newcommand{\Vix}{\vec{\boldsymbol \imath}}
\newcommand{\Vjx}{\vec{\boldsymbol \jmath}}
\newcommand{\Vkx}{\vec{\mathbf{k}}}
\newcommand{\Vlx}{\vec{\mathbf{l}}}
\newcommand{\Vmx}{\vec{\mathbf{m}}}
\newcommand{\Vnx}{\vec{\mathbf{n}}}
\newcommand{\Vox}{\vec{\mathbf{o}}}
\newcommand{\Vpx}{\vec{\mathbf{p}}}
\newcommand{\Vqx}{\vec{\mathbf{q}}}
\newcommand{\Vrx}{\vec{\mathbf{r}}}
\newcommand{\Vsx}{\vec{\mathbf{s}}}
\newcommand{\Vtx}{\vec{\mathbf{t}}}
\newcommand{\Vux}{\vec{\mathbf{u}}}
\newcommand{\Vvx}{\vec{\mathbf{v}}}
\newcommand{\Vwx}{\vec{\mathbf{w}}}
\newcommand{\Vxx}{\vec{\mathbf{x}}}
\newcommand{\Vyx}{\vec{\mathbf{y}}}
\newcommand{\Vzx}{\vec{\mathbf{z}}}

% Small characters with an arrow on top

\newcommand{\ax}{\vec{a}}
\newcommand{\bx}{\vec{b}}
\newcommand{\cx}{\vec{c}}
\newcommand{\dx}{\vec{d}}
\newcommand{\ex}{\vec{e}}
\newcommand{\fx}{\vec{f}}
\newcommand{\gx}{\vec{g}}
\newcommand{\hx}{\vec{h}}
\newcommand{\ix}{\vec{\imath}}
\newcommand{\jx}{\vec{\jmath}}
\newcommand{\kx}{\vec{k}}
\newcommand{\lx}{\vec{l}}
\newcommand{\mx}{\vec{m}}
\newcommand{\nx}{\vec{n}}
\newcommand{\ox}{\vec{o}}
%\newcommand{\px}{\vec{p}}
\newcommand{\qx}{\vec{q}}
\newcommand{\rx}{\vec{r}}
\newcommand{\sx}{\vec{s}}
\newcommand{\tx}{\vec{t}}
\newcommand{\ux}{\vec{u}}
\newcommand{\vx}{\vec{v}}
\newcommand{\wx}{\vec{w}}
\newcommand{\xx}{\vec{x}}
\newcommand{\yx}{\vec{y}}
\newcommand{\zx}{\vec{z}}
\newcommand{\vpsi}{\vec{\psi}}
\newcommand{\vphi}{\vec{\varphi}}
\newcommand{\vbeta}{\vec{\beta}}
\newcommand{\valpha}{\vec{\alpha}}
% Capital bold Characters

\newcommand{\VA}{{\mathbf{A}}}
\newcommand{\VB}{{\mathbf{B}}}
\newcommand{\VC}{{\mathbf{C}}}
\newcommand{\VD}{{\mathbf{D}}}
\newcommand{\VE}{{\mathbf{E}}}
\newcommand{\VF}{{\mathbf{F}}}
\newcommand{\VG}{{\mathbf{G}}}
\newcommand{\VH}{{\mathbf{H}}}
\newcommand{\VI}{{\mathbf{I}}}
\newcommand{\VJ}{{\mathbf{J}}}
\newcommand{\VK}{{\mathbf{K}}}
\newcommand{\VL}{{\mathbf{L}}}
\newcommand{\VM}{{\mathbf{M}}}
\newcommand{\VN}{{\mathbf{N}}}
\newcommand{\VO}{{\mathbf{O}}}
\newcommand{\VP}{{\mathbf{P}}}
\newcommand{\VQ}{{\mathbf{Q}}}
\newcommand{\VR}{{\mathbf{R}}}
\newcommand{\VS}{{\mathbf{S}}}
\newcommand{\VT}{{\mathbf{T}}}
\newcommand{\VU}{{\mathbf{U}}}
\newcommand{\VV}{{\mathbf{V}}}
\newcommand{\VW}{{\mathbf{W}}}
\newcommand{\VX}{{\mathbf{X}}}
\newcommand{\VY}{{\mathbf{Y}}}
\newcommand{\VZ}{{\mathbf{Z}}}

% Vektoren aus FE Raeumen

\newcommand{\Vah}{{{\mathbf{a}}_h}}
\newcommand{\Vbh}{{{\mathbf{b}}_h}}
\newcommand{\Vch}{{{\mathbf{c}}_h}}
\newcommand{\Vdh}{{{\mathbf{d}}_h}}
\newcommand{\Veh}{{{\mathbf{e}}_h}}
\newcommand{\Vfh}{{{\mathbf{f}}_h}}
\newcommand{\Vgh}{{{\mathbf{g}}_h}}
\newcommand{\Vhh}{{{\mathbf{h}}_h}}
\newcommand{\Vih}{{{\mathbf{i}}_h}}
\newcommand{\Vjh}{{{\mathbf{j}}_h}}
\newcommand{\Vkh}{{{\mathbf{k}}_h}}
\newcommand{\Vlh}{{{\mathbf{l}}_h}}
\newcommand{\Vmh}{{{\mathbf{m}}_h}}
\newcommand{\Vnh}{{{\mathbf{n}}_h}}
\newcommand{\Voh}{{{\mathbf{o}}_h}}
\newcommand{\Vph}{{{\mathbf{p}}_h}}
\newcommand{\Vqh}{{{\mathbf{q}}_h}}
\newcommand{\Vrh}{{{\mathbf{r}}_h}}
\newcommand{\Vsh}{{{\mathbf{s}}_h}}
\newcommand{\Vth}{{{\mathbf{t}}_h}}
\newcommand{\Vuh}{{{\mathbf{u}}_h}}
\newcommand{\Vvh}{{{\mathbf{v}}_h}}
\newcommand{\Vwh}{{{\mathbf{w}}_h}}
\newcommand{\Vxh}{{{\mathbf{x}}_h}}
\newcommand{\Vyh}{{{\mathbf{y}}_h}}
\newcommand{\Vzh}{{{\mathbf{z}}_h}}

% amstex bold symbols

\newcommand{\alphabf}{\boldsymbol \alpha}
\newcommand{\betabf}{\boldsymbol \beta}
\newcommand{\gammabf}{\boldsymbol \gamma}
\newcommand{\deltabf}{\boldsymbol \delta}
\newcommand{\epsilonbf}{\boldsymbol \epsilon}
\newcommand{\varepsilonbf}{\boldsymbol \varepsilon}
\newcommand{\zetabf}{\boldsymbol \zeta}
\newcommand{\etabf}{\boldsymbol \eta}
\newcommand{\thetabf}{\boldsymbol \theta}
\newcommand{\varthetabf}{\boldsymbol \vartheta}
\newcommand{\iotabf}{\boldsymbol \iota}
\newcommand{\kappabf}{\boldsymbol \kappa}
\newcommand{\lambdabf}{\boldsymbol \lambda}
\newcommand{\mubf}{\boldsymbol \mu}
\newcommand{\nubf}{\boldsymbol \nu}
\newcommand{\xibf}{\boldsymbol \xi}
\newcommand{\pibf}{\boldsymbol \pi}
\newcommand{\varpibf}{\boldsymbol \varpi}
\newcommand{\rhobf}{\boldsymbol \rho}
\newcommand{\varrhobf}{\boldsymbol \varrho}
\newcommand{\sigmabf}{\boldsymbol \sigma}
\newcommand{\varsigmabf}{\boldsymbol \varsigma}
\newcommand{\taubf}{\boldsymbol \tau}
\newcommand{\upsilonbf}{\boldsymbol \upsilon}
\newcommand{\phibf}{\boldsymbol \phi}
\newcommand{\varphibf}{\boldsymbol \varphi}
\newcommand{\chibf}{\boldsymbol \chi}
\newcommand{\psibf}{\boldsymbol \psi}
\newcommand{\omegabf}{\boldsymbol \omega}
\newcommand{\Gammabf}{\boldsymbol \Gamma}
\newcommand{\Deltabf}{\boldsymbol \Delta}
\newcommand{\Thetabf}{\boldsymbol \Theta}
\newcommand{\Lambdabf}{\boldsymbol \Lambda}
\newcommand{\Xibf}{\boldsymbol \Xi}
\newcommand{\Pibf}{\boldsymbol \Pi}
\newcommand{\Psibf}{\boldsymbol \Psi}
\newcommand{\Sigmabf}{\boldsymbol \Sigma}
\newcommand{\Upsilonbf}{\boldsymbol \Upsilon}
\newcommand{\Phibf}{\boldsymbol \Phi}
\newcommand{\Omegabf}{\boldsymbol \Omega}

% Roman capital letters

\newcommand{\Amat}{{\rm A}}
\newcommand{\Bmat}{{\rm B}}
\newcommand{\Cmat}{{\rm C}}
\newcommand{\Dmat}{{\rm D}}
\newcommand{\Emat}{{\rm E}}
\newcommand{\Fmat}{{\rm F}}
\newcommand{\Gmat}{{\rm G}}
\newcommand{\Hmat}{{\rm H}}
\newcommand{\Imat}{{\rm I}}
\newcommand{\Jmat}{{\rm J}}
\newcommand{\Kmat}{{\rm K}}
\newcommand{\Lmat}{{\rm L}}
\newcommand{\Mmat}{{\rm M}}
\newcommand{\Nmat}{{\rm N}}
\newcommand{\Omat}{{\rm O}}
\newcommand{\Pmat}{{\rm P}}
\newcommand{\Qmat}{{\rm Q}}
\newcommand{\Rmat}{{\rm R}}
\newcommand{\Smat}{{\rm S}}
\newcommand{\Tmat}{{\rm T}}
\newcommand{\Umat}{{\rm U}}
\newcommand{\Vmat}{{\rm V}}
\newcommand{\Wmat}{{\rm W}}
\newcommand{\Xmat}{{\rm X}}
\newcommand{\Ymat}{{\rm Y}}
\newcommand{\Zmat}{{\rm Z}}

% Kalligraphische Buchstaben

\newcommand{\Ca}{{\cal A}}
\newcommand{\Cb}{{\cal B}}
\newcommand{\Cc}{{\cal C}}
\newcommand{\Cd}{{\cal D}}
\newcommand{\Ce}{{\cal E}}
\newcommand{\Cf}{{\cal F}}
\newcommand{\Cg}{{\cal G}}
\newcommand{\Ch}{{\cal H}}
\newcommand{\Ci}{{\cal I}}
\newcommand{\Cj}{{\cal J}}
\newcommand{\Ck}{{\cal K}}
\newcommand{\Cl}{{\cal L}}
\newcommand{\Cm}{{\cal M}}
\newcommand{\Cn}{{\cal N}}
\newcommand{\Co}{{\cal O}}
\newcommand{\Cp}{{\cal P}}
\newcommand{\Cq}{{\cal Q}}
\newcommand{\Cr}{{\cal R}}
\newcommand{\Cs}{{\cal S}}
\newcommand{\Ct}{{\cal T}}
\newcommand{\Cu}{{\cal U}}
\newcommand{\Cv}{{\cal V}}
\newcommand{\Cw}{{\cal W}}
\newcommand{\Cx}{{\cal X}}
\newcommand{\Cy}{{\cal Y}}
\newcommand{\Cz}{{\cal Z}}

% Kalligraphische Buchstaben bold

\newcommand{\Cav}{\boldsymbol {\cal A}}
\newcommand{\Cbv}{\boldsymbol {\cal B}}
\newcommand{\Ccv}{\boldsymbol {\cal C}}
\newcommand{\Cdv}{\boldsymbol {\cal D}}
\newcommand{\Cev}{\boldsymbol {\cal E}}
\newcommand{\Cfv}{\boldsymbol {\cal F}}
\newcommand{\Cgv}{\boldsymbol {\cal G}}
\newcommand{\Chv}{\boldsymbol {\cal H}}
\newcommand{\Civ}{\boldsymbol {\cal I}}
\newcommand{\Cjv}{\boldsymbol {\cal J}}
\newcommand{\Ckv}{\boldsymbol {\cal K}}
\newcommand{\Clv}{\boldsymbol {\cal L}}
\newcommand{\Cmv}{\boldsymbol {\cal M}}
\newcommand{\Cnv}{\boldsymbol {\cal N}}
\newcommand{\Cov}{\boldsymbol {\cal O}}
\newcommand{\Cpv}{\boldsymbol {\cal P}}
\newcommand{\Cqv}{\boldsymbol {\cal Q}}
\newcommand{\Crv}{\boldsymbol {\cal R}}
\newcommand{\Csv}{\boldsymbol {\cal S}}
\newcommand{\Ctv}{\boldsymbol {\cal T}}
\newcommand{\Cuv}{\boldsymbol {\cal U}}
\newcommand{\Cvv}{\boldsymbol {\cal V}}
\newcommand{\Cwv}{\boldsymbol {\cal W}}
\newcommand{\Cxv}{\boldsymbol {\cal X}}
\newcommand{\Cyv}{\boldsymbol {\cal Y}}
\newcommand{\Czv}{\boldsymbol {\cal Z}}

% Kalligraphische Bucjstaben mit Subscript h

\newcommand{\Cah}{{\cal A}_h}
\newcommand{\Cbh}{{\cal B}_h}
\newcommand{\Cch}{{\cal C}_h}
\newcommand{\Cdh}{{\cal D}_h}
\newcommand{\Ceh}{{\cal E}_h}
\newcommand{\Cfh}{{\cal F}_h}
\newcommand{\Cgh}{{\cal G}_h}
\newcommand{\Chh}{{\cal H}_h}
\newcommand{\Cih}{{\cal I}_h}
\newcommand{\Cjh}{{\cal J}_h}
\newcommand{\Ckh}{{\cal K}_h}
\newcommand{\Clh}{{\cal L}_h}
\newcommand{\Cmh}{{\cal M}_h}
\newcommand{\Cnh}{{\cal N}_h}
\newcommand{\Coh}{{\cal O}_h}
\newcommand{\Cph}{{\cal P}_h}
\newcommand{\Cqh}{{\cal Q}_h}
\newcommand{\Crh}{{\cal R}_h}
\newcommand{\Csh}{{\cal S}_h}
\newcommand{\Cth}{{\cal T}_h}
\newcommand{\Cuh}{{\cal U}_h}
\newcommand{\Cvh}{{\cal V}_h}
\newcommand{\Cwh}{{\cal W}_h}
\newcommand{\Cxh}{{\cal X}_h}
\newcommand{\Cyh}{{\cal Y}_h}
\newcommand{\Czh}{{\cal Z}_h}

% Kalligraphische Buchstaben bold mit subscript h

\newcommand{\Cavh}{{\boldsymbol {\cal A}}_h}
\newcommand{\Cbvh}{{\boldsymbol {\cal B}}_h}
\newcommand{\Ccvh}{{\boldsymbol {\cal C}}_h}
\newcommand{\Cdvh}{{\boldsymbol {\cal D}}_h}
\newcommand{\Cevh}{{\boldsymbol {\cal E}}_h}
\newcommand{\Cfvh}{{\boldsymbol {\cal F}}_h}
\newcommand{\Cgvh}{{\boldsymbol {\cal G}}_h}
\newcommand{\Chvh}{{\boldsymbol {\cal H}}_h}
\newcommand{\Civh}{{\boldsymbol {\cal I}}_h}
\newcommand{\Cjvh}{{\boldsymbol {\cal J}}_h}
\newcommand{\Ckvh}{{\boldsymbol {\cal K}}_h}
\newcommand{\Clvh}{{\boldsymbol {\cal L}}_h}
\newcommand{\Cmvh}{{\boldsymbol {\cal M}}_h}
\newcommand{\Cnvh}{{\boldsymbol {\cal N}}_h}
\newcommand{\Covh}{{\boldsymbol {\cal O}}_h}
\newcommand{\Cpvh}{{\boldsymbol {\cal P}}_h}
\newcommand{\Cqvh}{{\boldsymbol {\cal Q}}_h}
\newcommand{\Crvh}{{\boldsymbol {\cal R}}_h}
\newcommand{\Csvh}{{\boldsymbol {\cal S}}_h}
\newcommand{\Ctvh}{{\boldsymbol {\cal T}}_h}
\newcommand{\Cuvh}{{\boldsymbol {\cal U}}_h}
\newcommand{\Cvvh}{{\boldsymbol {\cal V}}_h}
\newcommand{\Cwvh}{{\boldsymbol {\cal W}}_h}
\newcommand{\Cxvh}{{\boldsymbol {\cal X}}_h}
\newcommand{\Cyvh}{{\boldsymbol {\cal Y}}_h}
\newcommand{\Czvh}{{\boldsymbol {\cal Z}}_h}

%Vektorraumnormen

\newcommand{\NCa}[1]{{\left\|{#1}\right\|}_{\cal A}}
\newcommand{\NCb}[1]{{\left\|{#1}\right\|}_{\cal B}}
\newcommand{\NCc}[1]{{\left\|{#1}\right\|}_{\cal C}}
\newcommand{\NCd}[1]{{\left\|{#1}\right\|}_{\cal D}}
\newcommand{\NCe}[1]{{\left\|{#1}\right\|}_{\cal E}}
\newcommand{\NCf}[1]{{\left\|{#1}\right\|}_{\cal F}}
\newcommand{\NCg}[1]{{\left\|{#1}\right\|}_{\cal G}}
\newcommand{\NCh}[1]{{\left\|{#1}\right\|}_{\cal H}}
\newcommand{\NCi}[1]{{\left\|{#1}\right\|}_{\cal I}}
\newcommand{\NCj}[1]{{\left\|{#1}\right\|}_{\cal J}}
\newcommand{\NCk}[1]{{\left\|{#1}\right\|}_{\cal K}}
\newcommand{\NCl}[1]{{\left\|{#1}\right\|}_{\cal L}}
\newcommand{\NCm}[1]{{\left\|{#1}\right\|}_{\cal M}}
\newcommand{\NCn}[1]{{\left\|{#1}\right\|}_{\cal N}}
\newcommand{\NCo}[1]{{\left\|{#1}\right\|}_{\cal O}}
\newcommand{\NCp}[1]{{\left\|{#1}\right\|}_{\cal P}}
\newcommand{\NCq}[1]{{\left\|{#1}\right\|}_{\cal Q}}
\newcommand{\NCr}[1]{{\left\|{#1}\right\|}_{\cal R}}
\newcommand{\NCs}[1]{{\left\|{#1}\right\|}_{\cal S}}
\newcommand{\NCt}[1]{{\left\|{#1}\right\|}_{\cal T}}
\newcommand{\NCu}[1]{{\left\|{#1}\right\|}_{\cal U}}
\newcommand{\NCv}[1]{{\left\|{#1}\right\|}_{\cal V}}
\newcommand{\NCw}[1]{{\left\|{#1}\right\|}_{\cal W}}
\newcommand{\NCx}[1]{{\left\|{#1}\right\|}_{\cal X}}
\newcommand{\NCy}[1]{{\left\|{#1}\right\|}_{\cal Y}}
\newcommand{\NCz}[1]{{\left\|{#1}\right\|}_{\cal Z}}

% Blackboard bold characters

\newcommand{\bbA}{\mathbb{A}}
\newcommand{\bbB}{\mathbb{B}}
\newcommand{\bbC}{\mathbb{C}}
\newcommand{\bbD}{\mathbb{D}}
\newcommand{\bbE}{\mathbb{E}}
\newcommand{\bbF}{\mathbb{F}}
\newcommand{\bbG}{\mathbb{G}}
\newcommand{\bbH}{\mathbb{H}}
\newcommand{\bbI}{\mathbb{I}}
\newcommand{\bbJ}{\mathbb{J}}
\newcommand{\bbK}{\mathbb{K}}
\newcommand{\bbL}{\mathbb{L}}
\newcommand{\bbM}{\mathbb{M}}
\newcommand{\bbN}{\mathbb{N}}
\newcommand{\bbO}{\mathbb{O}}
\newcommand{\bbP}{\mathbb{P}}
\newcommand{\bbQ}{\mathbb{Q}}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbS}{\mathbb{S}}
\newcommand{\bbT}{\mathbb{T}}
\newcommand{\bbU}{\mathbb{U}}
\newcommand{\bbV}{\mathbb{V}}
\newcommand{\bbW}{\mathbb{W}}
\newcommand{\bbX}{\mathbb{X}}
\newcommand{\bbY}{\mathbb{Y}}
\newcommand{\bbZ}{\mathbb{Z}}


% Euler
\newcommand{\FA}{\mathfrak{A}}
\newcommand{\FB}{\mathfrak{B}}
\newcommand{\FC}{\mathfrak{C}}
\newcommand{\FD}{\mathfrak{D}}
\newcommand{\FE}{\mathfrak{E}}
\newcommand{\FF}{\mathfrak{F}}
\newcommand{\FG}{\mathfrak{G}}
\newcommand{\FH}{\mathfrak{H}}
\newcommand{\FI}{\mathfrak{I}}
\newcommand{\FJ}{\mathfrak{J}}
\newcommand{\FK}{\mathfrak{K}}
\newcommand{\FL}{\mathfrak{L}}
\newcommand{\FM}{\mathfrak{M}}
\newcommand{\FN}{\mathfrak{N}}
\newcommand{\FO}{\mathfrak{O}}
\newcommand{\FP}{\mathfrak{P}}
\newcommand{\FQ}{\mathfrak{Q}}
\newcommand{\FR}{\mathfrak{R}}
\newcommand{\FS}{\mathfrak{S}}
\newcommand{\FT}{\mathfrak{T}}
\newcommand{\FU}{\mathfrak{U}}
\newcommand{\FV}{\mathfrak{V}}
\newcommand{\FW}{\mathfrak{W}}
\newcommand{\FX}{\mathfrak{X}}
\newcommand{\FY}{\mathfrak{Y}}
\newcommand{\FZ}{\mathfrak{Z}}

\newcommand{\Fa}{\mathfrak{a}}
\newcommand{\Fb}{\mathfrak{b}}
\newcommand{\Fc}{\mathfrak{c}}
\newcommand{\Fd}{\mathfrak{d}}
\newcommand{\Fe}{\mathfrak{e}}
\newcommand{\Ff}{\mathfrak{f}}
\newcommand{\Fg}{\mathfrak{g}}
\newcommand{\Fh}{\mathfrak{h}}
\newcommand{\Fi}{\mathfrak{i}}
\newcommand{\Fj}{\mathfrak{j}}
\newcommand{\Fk}{\mathfrak{k}}
\newcommand{\Fl}{\mathfrak{l}}
\newcommand{\Fm}{\mathfrak{m}}
\newcommand{\Fn}{\mathfrak{n}}
\newcommand{\Fo}{\mathfrak{o}}
\newcommand{\Fp}{\mathfrak{p}}
\newcommand{\Fq}{\mathfrak{q}}
\newcommand{\Fr}{\mathfrak{r}}
\newcommand{\Fs}{\mathfrak{s}}
\newcommand{\Ft}{\mathfrak{t}}
\newcommand{\Fu}{\mathfrak{u}}
\newcommand{\Fv}{\mathfrak{v}}
\newcommand{\Fw}{\mathfrak{w}}
\newcommand{\Fx}{\mathfrak{x}}
\newcommand{\Fy}{\mathfrak{y}}
\newcommand{\Fz}{\mathfrak{z}}

%Cross product of vectors in R^3
\newcommand{\cross}[2]{{#1}\times{#2}}

%shortcut for citations done prior
\newcommand{\oc}{\textit{op. cit.} }

%shortcut for very common expressions
\newcommand{\ocf}{ \ensuremath{\frac{\omega}{c} } }
\newcommand{\rocf}{ \ensuremath{\frac{r\omega}{c} } }
\newcommand{\ul}[1]{\ensuremath{\underline{#1}}}
